Unique Identification of Macaques for Population Monitoring and Control

Despite loss of natural habitat due to development and urbanization, certain species like the Rhesus macaque have adapted well to the urban environment. With abundant food and no predators, macaque populations have increased substantially in urban areas, leading to frequent conflicts with humans. Overpopulated areas often witness macaques raiding crops, feeding on bird and snake eggs as well as destruction of nests, thus adversely affecting other species in the ecosystem. In order to mitigate these adverse effects, sterilization has emerged as a humane and effective way of population control of macaques. As sterilization requires physical capture of individuals or groups, their unique identification is integral to such control measures. In this work, we propose the Macaque Face Identification (MFID), an image based, non-invasive tool that relies on macaque facial recognition to identify individuals, and can be used to verify if they are sterilized. Our primary contribution is a robust facial recognition and verification module designed for Rhesus macaques, but extensible to other non-human primate species. We evaluate the performance of MFID on a dataset of 93 monkeys under closed set, open set and verification evaluation protocols. Finally, we also report state of the art results when evaluating our proposed model on endangered primate species.

==> Sections/Discussion.tex <==
We developed MFID an automated non-invasive approach for uniquely identifying Rhesus macaques from camera captured images. The developed system holds relevance to biologists as well as conservationist due to the following reasons. For Rhesus macaques, database can be put in place by crowd sourcing, as these primate dwell in urban setting. This would aid in monitoring both, the effectiveness of population control measures like sterilization and population assessment. Another, extension of proposed MFID system is to aid the field visits to capture monkeys for sterilization and avoid recapture of already sterilized monkey by identifying the status with a application installed in their handheld devices. Therefore, in order to achieve this extensibility, we employed a DenseNet-121 network that takes only   $28.4$  MB of memory as oppose to other models like AlexNet, Resnet-50 and ResNet-18 that occupy 245 MB, 90 MB and 44 MB respectively. Furthermore, it is not limited to Rhesus macaques, state of the art results on endangered species like chimpanzees show that the application is a possible solution for detecting illegally traded as well as escaped species.


==> Sections/tsne.tex <==

\begin{figure*}[h]
% \vspace{-0.5cm}	
	\centering
			\subfigure[C-Zoo+C-Tai]{\includegraphics[trim=2cm 1cm 2cm 1cm,clip=true,width =0.24\textwidth,scale=1]{plots/test_ds121_ctai_zoo_sm.jpg} \includegraphics[trim=2cm 1cm 2cm 1cm,clip=true,width  =0.24\textwidth,scale=1]{plots/test_ds121_ctai_zoo_kldiv.jpg}}
%         \subfigure[C-Zoo+C-Tai]{\includegraphics[width  =0.235\textwidth,scale=1]{plots/test_ds121_ctai_zoo_kldiv.jpg} }
        \subfigure[Rhesus Macaques]{ \includegraphics[trim=2cm 1cm 2cm 1cm,clip=true, width  =0.24\textwidth,scale=1]{plots/test_ds121_all_maca_sm.jpg}\includegraphics[trim=2cm 1cm 2cm 1cm,clip=true, width  =0.24\textwidth,scale=1]{plots/test_ds121_all_maca_kldiv.jpg}}
%              \subfigure[Rhesus Macaques]{ \includegraphics[width  =0.235\textwidth,scale=1]{plots/test_ds121_all_maca_kldiv.jpg}}
%         {\includegraphics[width =40mm,scale=0.8]{Figures/cmu_recon.png} 
%         \includegraphics[width =40mm,scale=0.8]{Figures/54_recon.png}}
		\caption{ Visualization of features learned with cross entropy loss (Left) and MFID loss (Right) for (a) C-Zoo+C-Tai and (b) Rhesus Macaques dataset}
		\label{fig: tsne}
%         \vspace{-0.5cm}	
\end{figure*}
